Revisiting Cross-Lingual Summarization: A Corpus-based Study and A New Benchmark with Improved Annotation

Most existing cross-lingual summarization (CLS) work constructs CLS corpora by simply and directly translating pre-annotated summaries from one language to another, which can contain errors from both summarization and translation processes. To address this issue, we propose ConvSumX, a cross-lingual conversation summarization benchmark, through a new annotation schema that explicitly considers source input context. ConvSumX consists of 2 sub-tasks under different real-world scenarios, with each covering 3 language directions. We conduct thorough analysis on ConvSumX and 3 widely-used manually annotated CLS corpora and empirically find that ConvSumX is more faithful towards input text. Additionally, based on the same intuition, we propose a 2-Step method, which takes both conversation and summary as input to simulate human annotation process. Experimental results show that 2-Step method surpasses strong baselines on ConvSumX under both automatic and human evaluation. Analysis shows that both source input text and summary are crucial for modeling cross-lingual summaries.

==> case1.tex <==
% \begin{table*}[h]
% \renewcommand{\arraystretch}{1.5}
%     \centering
%     \small
%     \begin{tabular}{lr|p{13cm}}
%     \thickhline
%     \multicolumn{3}{c}{\textbf{\emph{DialogSumX}}}\\
%     \thickhline
%         \multicolumn{2}{l|}{Input Text}  & \#Person1\#: Ms. Dawson, I need you to take a dictation for me. \#Person2\#: Yes, sir... \#Person1\#: This should go out as an intra-office memorandum to all employees by this afternoon. Are you ready? \#Person2\#: Yes, sir. Go ahead. \#Person1\#: Attention all staff... Effective immediately, all office communications are restricted to email correspondence and official memos. The use of Instant Message programs by employees during working hours is strictly prohibited. \#Person2\#: Sir, does this apply to intra-office communications only? Or will it also restrict external communications? \#Person1\#: It should apply to all communications, not only in this office between employees, but also any outside communications. \#Person2\#: But sir, many employees use Instant Messaging to communicate with their clients. \#Person1\#: They will just have to change their communication methods. I don't want any - one using Instant Messaging in this office. It wastes too much time! Now, please continue with the memo. Where were we? \#Person2\#: This applies to internal and external communications. \#Person1\#: Yes. Any employee who persists in using Instant Messaging will first receive a warning and be placed on probation. At second offense, the employee will face termination. Any questions regarding this new policy may be directed to department heads. \#Person2\#: Is that all? \#Person1\#: Yes. Please get this memo typed up and distributed to all employees before 4 pm.  \\
%         \hline
%         \multirow{3}{*}{\emph{S-T}} & En2Zh & \begin{CJK}{UTF8}{gbsn}\small{论文(academic paper)/讲述(talk)/...}\end{CJK} \\
%         \cline{3-3}
%          & En2Fr & \\
%         \cline{3-3}
%         \hline
%         \multirow{3}{*}{2-Step} & En2Zh & \\
%         \cline{3-3}
%          & En2Fr & \\
%         \cline{3-3}
%          & En2Ukr & \\
%         \hline
%         \multirow{3}{*}{Gold} & En2Zh & \\
%         \cline{3-3}
%          & En2Fr & \\
%         \cline{3-3}
%          & En2Ukr & \\
%     \thickhline
%     \end{tabular}
%     \caption{Case study (b): Gold and generated summaries by 100-shot PEGASUS and \textsc{UniSumm} on MultiNews, respectively.
%     ``|||||'' seperates different reports in the input. }
%     \label{tab:case_multinews}
% \end{table*}

==> case2.tex <==
\begin{table*}[h]
\renewcommand{\arraystretch}{1.5}
    \centering
    \small
    \begin{tabular}{lr|p{13cm}}
    \thickhline
    \multicolumn{3}{c}{\textbf{\emph{QMSumX}}}\\
    \thickhline
        \multicolumn{2}{l|}{Input Text}  & \#Person1\#: Ms. Dawson, I need you to take a dictation for me. \#Person2\#: Yes, sir... \#Person1\#: This should go out as an intra-office memorandum to all employees by this afternoon. Are you ready? \#Person2\#: Yes, sir. Go ahead. \#Person1\#: Attention all staff... Effective immediately, all office communications are restricted to email correspondence and official memos. The use of Instant Message programs by employees during working hours is strictly prohibited. \#Person2\#: Sir, does this apply to intra-office communications only? Or will it also restrict external communications? \#Person1\#: It should apply to all communications, not only in this office between employees, but also any outside communications. \#Person2\#: But sir, many employees use Instant Messaging to communicate with their clients. \#Person1\#: They will just have to change their communication methods. I don't want any - one using Instant Messaging in this office. It wastes too much time! Now, please continue with the memo. Where were we? \#Person2\#: This applies to internal and external communications. \#Person1\#: Yes. Any employee who persists in using Instant Messaging will first receive a warning and be placed on probation. At second offense, the employee will face termination. Any questions regarding this new policy may be directed to department heads. \#Person2\#: Is that all? \#Person1\#: Yes. Please get this memo typed up and distributed to all employees before 4 pm.  \\
        \hline
        \multirow{3}{*}{\emph{S-T}} & En2Zh & \\
        \cline{3-3}
         & En2Fr & \\
        \cline{3-3}
         & En2Ukr & \\
        \hline
        \multirow{3}{*}{2-Step} & En2Zh & \\
        \cline{3-3}
         & En2Fr & \\
        \cline{3-3}
         & En2Ukr & \\
        \hline
        \multirow{3}{*}{Gold} & En2Zh & \\
        \cline{3-3}
         & En2Fr & \\
        \cline{3-3}
         & En2Ukr & \\
    \thickhline
    \end{tabular}
    \caption{Case study (b): Gold and generated summaries by 100-shot PEGASUS and \textsc{UniSumm} on MultiNews, respectively.
    ``|||||'' seperates different reports in the input. }
    \label{tab:case_multinews}
\end{table*}

==> error_cases.tex <==

\begin{table*}[h]
\renewcommand{\arraystretch}{1.5}
    \centering
    \small
    \begin{tabular}{l|p{13.5cm}}
    \thickhline
    \multicolumn{2}{c}{\textbf{Word Sense}}\\
    \thickhline
        dataset & NCLS EN2ZH\\
        
        \hline
        Input text  & America is on high alert for terrorist threats after a string of incidents including two flights to Paris being diverted by bomb threats, a Muslim family being ejected from a Baltimore plane, a bomb squad being called to a Chicago airport and a Disney resort being evacuated because of a bomb scare. Air France Flight 55 from Washington s Dulles International Airport to Charles de Gaulle Airport in Paris was diverted to an airport in Halifax, Nova Scotia, reports CNN, after a bomb threat was called in from the ground on Tuesday night. While Flight 65, headed from Los Angeles to Paris, was diverted to Salt Lake City. Both flights landed safely and are being investigated by the FBI. Then on Tuesday evening, Disney All Star Movies Resort in Orlando, Florida, was briefly evacuated due to an unspecified bomb threat......    \\
        \hline
        {En summary} & Bomb squad \textcolor{red}{called to} Chicago's O'Hare airport for suspicious package .
        \\
        \hline
        \multirow{2}{*}{Zh summary}  & \begin{CJK}{UTF8}{gbsn}\small{拆弹小组\textcolor{red}{打电话到}芝加哥奥黑尔机场索要“可疑”包裹。}\end{CJK} \\ 
        & (Bomb squad \textcolor{red}{made a phone call to} Chicago's O'Hare airport for suspicious package.)
        \\
        \hline
        dataset & XSAMSum\\
        
        \hline
        Input text  & Mika: I wanted to ask you to stop supporting the queer group Ann: why? I think they do great things Mika: they discriminated Molly horribly Ann: why? how? Mika: they refused to include her in the panel about sexuality Tom: did they give a reason? Mika: they said her research doesn't match the topic of the panel, what is a bullshit Mika: I believe it's only because she is straight Tom: hmm...   \\
        \hline
        {En summary} & \textcolor{red}{The queer group}  discriminated Molly - they refused to include her in the panel about sexuality.
        \\
        \hline
        \multirow{2}{*}{Zh summary} & \begin{CJK}{UTF8}{gbsn}\small{\textcolor{red}{同性恋团体}歧视莫莉——他们拒绝让她参加关于性的小组讨论。}\end{CJK}
        \\& (\textcolor{red}{The homosexuality group}  discriminated Molly - they refused to include her in the panel about sexuality.)
         % \hline{Translation of en summary} & 
        
        \\
        \hline
        dataset & XMediaSum40K\\
        
        \hline
        Input text  & ...... We should also note, and this will come up in a little bit, that Bakari is supporting Kamala Harris for president. Also with us, John Avlon, CNN senior political analyst. We have this august, political panel here to talk about soccer. Why? Because the U.S. soccer team is political. And I think proudly so. They're on their way back to the United States. Nancy Pelosi has invited them to Capitol Hill. What will the president do? He claims he hasn't even thought about whether he's inviting them to the White House. Listen.QUESTION: Will you invite the women's team to the White House, the soccer team?......    \\
        \hline
        {En summary} & U.S. Women's Soccer Team \textcolor{red}{Invited to} the White House
        \\
        \hline
        \multirow{2}{*}{Zh summary} & \begin{CJK}{UTF8}{gbsn}\small{美国女足\textcolor{red}{获邀入主}白宫。}\end{CJK}
        \\& (Women's Soccer Team \textcolor{red}{Invited to rule} the White House.)
        \\  
    \thickhline
     \multicolumn{2}{c}{\textbf{Terminology
}}\\
    \thickhline
     dataset & NCLS EN2ZH\\
     \hline
     Input text & Fred: A hard-right group connected to Thomas Mair is linked to the Brexit campaign, The Mail on Sunday can reveal. Our investigation has established that the racist Springbok Club, which once described Mair as one of its earliest subscribers and supporters, has sent newsletters to British members urging them to support the Leave campaign. The leaflets, all sent in the last three months, say: The Springbok Club is part of the Patriotic Forum, which moved from South Africa to Britain after the downfall of apartheid. Its newsletter in April said that the anti-EU Bruges Group had asked for help with a Vote Leave campaign centre it had set up in West London...... \\
     \hline
     {En summary}& Racist group has sent newsletters to British members \textcolor{red}{urging Leave vote} .\\
     \hline
     \multirow{2}{*}{Zh summary} & \begin{CJK}{UTF8}{gbsn}\small{种族主义团体向英国成员发送了时事通讯，敦促他们\textcolor{red}{投票离开}。}\end{CJK}  \\ 
     & ( Racist groups sent newsletters to British members \textcolor{red}{urging them to vote to leave}. )
        \\
        

     \thickhline
     dataset & XSAMSum\\
     \hline
     Input text & Fred: file photo Fred: Theoretically everything that has been posted online can be deleted Fred: But Internet doesn't forget :D George: On the one hand I admire your speed at downloading embarassing content George: On the other hand I really don't get it why are you doing this xD Fred: It's simple. When someone is a hypocrite and sometimes proves it with posting such content. I feel obliged to reveal his hypocrisy or ignorance. Fred: Take this politician. The print screen I sent you was a photo of his public post about coal miners 5 years ago. Fred: file photo  This one is from today. George: He contradicts himself...... \\
     \hline
     {En summary}& \textcolor{red}{Fed} shows Tom two photos revealing the hypocrisy of a politician on closing down the mines.\\
     \hline
     \multirow{2}{*}{Zh summary} & \begin{CJK}{UTF8}{gbsn}\small{\textcolor{red}{美联储}给汤姆看的两张照片揭露了一个政治家在关闭煤矿这件事上暴露的虚伪。}\end{CJK}  \\ 
     & (\textcolor{red}{Federal Reserve System} shows Tom two photos revealing the hypocrisy of a politician on closing down the mines.)
        \\
%       \thickhline


    
    \end{tabular}
    \caption{Case study (b): Gold and generated summaries by 100-shot PEGASUS and \textsc{UniSumm} on MultiNews, respectively.
    ``|||||'' seperates different reports in the input. }
    \label{tab:case_multinews}
\end{table*}



\begin{table*}[h]
\renewcommand{\arraystretch}{1.5}
    \centering
    \small
    \begin{tabular}{l|p{13.5cm}}
    \thickhline
     \multicolumn{2}{c}{\textbf{Coreference
}}\\
     \thickhline
     dataset & XSAMSum\\
     \hline
     Input text& Wanda: Let's make a party! Gina: Why? Wanda: beacuse. I want some fun! Gina: ok, what do u need? Wanda: 1st I need too make a list Gina: noted and then? Wanda: well, could u take yours father car and go do groceries with me? Gina: don't know if he'll agree Wanda: I know, but u can ask :) Gina: I'll try but theres no promisess Wanda: I know, u r the best! Gina: When u wanna go Wanda: Friday? Gina: ok, I'll ask"\\
    \hline
     {En summary} & Wanda wants to throw a party. She asks Gina to borrow her father's car and go do groceries together. They set \textcolor{red}{the date} for Friday. \\
     \hline
     \multirow{2}{*}{Zh summary}&\begin{CJK}{UTF8}{gbsn}\small{旺达想办个聚会。她问吉娜借她父亲的车，两人一起去买聚会用的东西。他们把\textcolor{red}{聚会的日期}定在了周五。}\end{CJK} \\
     & (Wanda wants to throw a party. She asks Gina to borrow her father's car and go do groceries together. They set \textcolor{red}{the date of party} for Friday.) 
        \\
     \thickhline
    dataset & NCLS en2zh\\
     \hline
     Input text&For Mark Cooper, the best phone call of Saturday night was one he made to his dad Terry. Not because he could tell him how his Swindon team had ended Bristol City unbeaten record. But because he could make it at all. Mark had spent the last international break at the hospital bedside in Tenerife where Terry, England \'s swashbuckling left back in the 1970 World Cup, was in intensive care following a life-or-death bowel cancer operation.  ...... \\
    \hline
     {En summary} &Cooper had been at hospital bedside of his dad in Tenerife after \textcolor{red}{he} underwent life-or-death bowel cancer operation .\\
    \hline
     \multirow{2}{*}{Zh summary}& \begin{CJK}{UTF8}{gbsn}\small{\textcolor{red}{库珀}在接受了生死攸关的肠癌手术后，一直在特内里费他父亲的医院床边。}\end{CJK}
     \\
     &(Cooper had been at hospital bedside of his dad in Tenerife after \textcolor{red}{Cooper} underwent life-or-death bowel cancer operation .)
     \\
     
    \multicolumn{2}{c}{\textbf{Sentence Relation
    }}\\
    \thickhline
    dataset & NCLS EN2ZH\\
    \hline
    Input text& ..... Silva was pictured nursing his problem at home ahead of the game, with a full diagnosis yet to be completed by PSG s medical team. Thiago Silva who is recuperating at home from a thigh injury and will miss Paris Saint-Germain's game at Nice . Silva was substituted in the defeat by Barcelona in midweek and the injury is still keeping him out ..... \\
    \hline
     {En summary} &   Brazilian defender had to substituted  \textcolor{red}{against Barcelona} in Champions League  \\
     \hline
     \multirow{2}{*}{Zh summary}&
     \begin{CJK}{UTF8}{gbsn}\small{巴西后卫}不得不在冠军联赛中替换\textcolor{red}{巴塞罗那}。\end{CJK}
     \\
     & Brazilian defender had to substituted \textcolor{red}{Barcelona} in Champions League 
     \\
    \thickhline
    dataset & XSAMSum\\
    \hline
    Input text& John: Ela i am coming in 10 mins please give me my walle outside t i forgot it Ela: yes just saw it when you are here call me John: but your phone is busy thats why i messaged keep it free please i am getting late Ela: oh yes was talking to mom ... its free now John: ok \\
    \hline
     {En summary} & John forgot his wallet. He wants Ela to \textcolor{red}{ give it to him outside in 10 minutes.} \\
     \hline
     \multirow{2}{*}{Zh summary}&
     \begin{CJK}{UTF8}{gbsn}\small{约翰忘了带钱包，他要艾拉\textcolor{red}{10分钟内给他送过来。}}\end{CJK}
     \\
     & (John forgot his wallet. He wants Ela to \textcolor{red}{bring it to him within 10 minutes.})
     \\
    
    
    \end{tabular}
    \caption{Case study (b): Gold and generated summaries by 100-shot PEGASUS and \textsc{UniSumm} on MultiNews, respectively.
    ``|||||'' seperates different reports in the input. }
    \label{tab:case_multinews2}
\end{table*}





\begin{table*}[h]
\renewcommand{\arraystretch}{1.5}
    \centering
    \small
    \begin{tabular}{l|p{13.5cm}}
    \thickhline
     
    \multicolumn{2}{c}{\textbf{Others
    }}\\
    \thickhline
    dataset & NCLS en2zh\\
    \hline
    Input text& Baby lobsters might not be able to survive in the ocean's waters if the ocean continues to warm at the expected rate. That is the key finding of a study performed by scientists in Maine, the state most closely associated with lobster....... \\
    \hline
     {En summary} & \textcolor{red}{Five degrees} is also \textcolor{red}{how much} Gulf of Maine is expected to \textcolor{red}{warm}  by 2100 . \\
     \hline
     \multirow{2}{*}{Zh summary}&
     \begin{CJK}{UTF8}{gbsn}\small{\textcolor{red}{五度}也是缅因湾到2100年的预期气温。}\end{CJK}
     \\
     & (\textcolor{red}{Five degrees} is also Gulf of Maine is expected to by 2100 .)
     \\
     \thickhline
    dataset & XSAMSum\\
    \hline
    Input text& Elliot: i can't talk rn, i'm rly busy Elliot: can i call u back in about 2 hours? Jordan: Not really, I'm going to a funeral. Jordan: I'll call you tonight, ok? Elliot: sure Elliot: whose funeral is it? Jordan: My colleague's, Brad. Jordan: I told you about him, he had a liver cancer. Elliot: i'm so sorry man, i hope u're ok Elliot: i'll call u at 8 pm \\
    \hline
     {En summary} & Elliot can't talk to Jordan now, he's busy. He'll call him back at \textcolor{red}{8} pm. Jordan is going to Brad's funeral. He had liver cancer. \\
     \hline
     \multirow{2}{*}{Zh summary}&
     \begin{CJK}{UTF8}{gbsn}\small{艾略特现在没空和乔丹说话，他很忙。晚上\textbf{\textcolor{red}{6}}点他会给乔丹回电话。乔丹要去参加布拉德的葬礼，布拉德因肝癌去世了。}\end{CJK}
     \\
     & (Elliot can't talk to Jordan now, he's busy. He'll call him back at \textcolor{red}{6} pm. Jordan is going to Brad's funeral. He had liver cancer.)
     \\

    
    \end{tabular}
    \caption{Case study (b): Gold and generated summaries by 100-shot PEGASUS and \textsc{UniSumm} on MultiNews, respectively.
    ``|||||'' seperates different reports in the input. }
    \label{tab:case_multinews2}
\end{table*}
